Weakly-Supervised 3D Medical Image Segmentation using Geometric Prior and Contrastive Similarity

Medical image segmentation is almost the most important pre-processing procedure in computer-aided diagnosis but is also a very challenging task due to the complex shapes of segments and various artifacts caused by medical imaging, (i.e., low-contrast tissues, and non-homogenous textures). In this paper, we propose a simple yet effective segmentation framework that incorporates the geometric prior and contrastive similarity into the weakly-supervised segmentation framework in a loss-based fashion. The proposed geometric prior built on point cloud provides meticulous geometry to the weakly-supervised segmentation proposal, which serves as better supervision than the inherent property of the bounding-box annotation (i.e., height and width). Furthermore, we propose contrastive similarity to encourage organ pixels to gather around in the contrastive embedding space, which helps better distinguish low-contrast tissues. The proposed contrastive embedding space can make up for the poor representation of the conventionally-used gray space. Extensive experiments are conducted to verify the effectiveness and the robustness of the proposed weakly-supervised segmentation framework. The proposed framework is superior to state-of-the-art weakly-supervised methods on the following publicly accessible datasets: LiTS 2017 Challenge, KiTS 2021 Challenge, and LPBA40. We also dissect our method and evaluate the performance of each component.

==> chap/abstract.tex <==
\begin{abstract}
Medical image segmentation is almost the most important pre-processing procedure in computer-aided diagnosis but is also a very challenging task due to the complex shapes of segments and various artifacts caused by medical imaging, ({\em i.e.}, low-contrast tissues, and non-homogenous textures). In this paper, we propose a simple yet effective segmentation framework that incorporates the geometric prior and contrastive similarity into the weakly-supervised segmentation framework in a loss-based fashion. The proposed geometric prior built on point cloud provides meticulous geometry to the weakly-supervised segmentation proposal, which serves as better supervision than the inherent property of the bounding-box annotation (\emph{i.e.}, height and width). Furthermore, we propose the contrastive similarity to encourage organ pixels to gather around in the contrastive embedding space, which helps better distinguish low-contrast tissues. The proposed contrastive embedding space can make up for the poor representation of the conventionally-used 
gray space. Extensive experiments are conducted to verify the effectiveness and the robustness of the proposed weakly-supervised segmentation framework. The proposed framework are superior to state-of-the-art weakly-supervised methods on the following publicly accessible datasets: LiTS 2017 Challenge, KiTS 2021 Challenge and LPBA40. We also dissect our method and evaluate the performance of each component.

\end{abstract}

==> chap/conclusion.tex <==
% \section{Discussion}
% Through extensive experiments, we successfully verify the effectiveness of introducing geometric prior into the training of the weakly-supervised segmentation framework. Furthermore, we propose the contrastive similarity to make up the poor representation of gray space due to the medical artifacts raised by the specific physical or technical issues in medical imaging area. We dissect our method and evaluate the effects of each components. The results consistently show the superiority of our proposed method over three widely-used medical segmentation datasets in terms of dice score. We then show the robustness of our proposed components by introducing into other framework ({\em i.e.,} DeepLabV3). By incorporating geometric prior and contrastive similarity into training loss, the segmentation framework is largely improved 9.7\% in terms of DSC (\%). Importantly, we also notice that the template supervise the proposal generation from the perspective of geometry shape and internal details. Ablations experiments are conducted to further analysis the effect of each aspect. We also demonstrate that previous works~\cite{huang2021medical} incorporating geometric prior often process images in 2D space. Instead, we convert the 3D medical image into point cloud 3D space and optimize the proposal generation in a 3D embedding space. This helps better capture the geometry shape of the template organ.

% This research will probably serve as a base research for possible future studies on incorporating geometry prior and contrastive similarity into the weakly-supervised segmentation framework, especially for medical image segmentation (considering the specific shape and position of the organ). Further study of combining geometric prior and contrastive similarity into the weakly-supervised segmentation is needed. In this work, we observe that organs usually have specific shape and position which can be further used as the prior to better supervise the training of the proposal generation. Furthermore, we observe that medical images have special medical artifacts ~\cite{budrys2018artifacts}. The low-contrast tissues and non-homogenous texture can be distinguished by the proposed contrastive head. The widely-used gray space perform poorly in medical images due to the fore-mentioned medical artifacts. We successfully learn the difference between organ pixels and non-organ pixels. To summarize, we propose a simple yet effective weakly-supervised segmentation framework, which can be easily applied to other weakly-supervised segmentation framework.The proposed geometric prior can better supervise the learning of the proposal, which helps build the completeness of the result. Furthermore, the proposed contrastive similarity can better represent the feature space than gray space, which contributes to the abundant details of the generated proposal.


% Our method consists of two major components to address \textit{\qone} and \textit{\qtwo} challenges, respectively. The first challenge is solved by our geometric prior, where proposals are constrained by a given template. The overall structure of the generated proposal will be optimized by minimizing the distance from a given template. This component ensures the geometry shape and internal structures of the proposal. The second component is the contrastive similarity, addressing the issues raised by medical image artifacts. By pre-training a contrastive head, we successfully learn the difference between organ pixels and non-organ pixels. This component can better distinguish low-contrast tissues and non-homogenous texture than conventionally widely-used gray space. Through extensive experiments, we demonstrate that our method can generate a high-quality segmentation proposal, along with abundant internal details and accurate boundaries. We show that our method outperforms other bounding-box weakly-supervised methods ~\cite{tian2021boxinst, kervadec2019constrained} under similar settings. We also conduct extensive experiments to verify the effectiveness of components in our method.

% In summary, we make three major contributions in this paper.
% \begin{itemize}
%     \item We propose a simple yet effective weakly-supervised segmentation framework, which can be easily applied to other weakly-supervised segmentation framework, \emph{i.e.}, DeepLabV3~\cite{chen2017rethinking}.
%     \item We propose the geometric prior to better guide the learning of the proposal, which helps build the completeness of the result.
%     \item The proposed contrastive similarity can better represent the feature space than color space, which contributes to the abundant details of the generated proposal.
% \end{itemize}
% Our code and data will be made publicly available for further research.

\section{Conclusion}
\label{sec:conclusion}
\IEEEPARstart{I}{n} this work, we propose a novel weakly-supervised segmentation framework with bounding-box annotations. We introduce the geometric prior and the contrastive similarity to address the challenges of \qone\ and \qtwo, enhancing the practicability and robustness of the weakly-supervised segmentation framework. The geometric prior enables the learning of delicate and complex structures, and the contrastive similarity helps better distinguish organ pixels from non-organ pixels. 

Our framework is general, which can be easily applied to many weakly-supervised segmentation models and thus improve their performances. It will probably serve as a base for possible future studies on weakly-supervised segmentation, especially for medical image segmentation on organs that are with a specific shape. Extensive experiments are conducted to verify the effectiveness and the superiority of our proposed geometric prior and contrastive similarity.




==> chap/exp.tex <==
\section{Experiments}
\label{sec:exp}

\subsection{Datasets}
\begin{itemize}
    \item LiTS: The public liver LiTS~\cite{bilic2019liver} dataset comprises 201 CT scans from various CT scanners and devices. The resolution of images in this dataset is from $0.56$mm to $1.0$mm in axial and 0.45mm to 6.0mm in $z$ direction. Slices in $z$ range from 42 to 1026. We split 131 cases into training and evaluation sets by a ratio of 4:1.
    \item KiTS21: The publicly accessible KiTS21~\cite{heller2020state} dataset consists of 300 cases during the period from 2010 to 2020. Each CT scan in the dataset is annotated by three expert annotators for the following semantic classes: Kidney, Tumor, and Cyst. We split the provided CT scans into training and validation sets by a ratio of 4:1. 
    \item LPBA40: This dataset consists of 40 T1-weighted image volumes from randomly selected cases (among 40 scans: 20 males, 20 females, and 29.2 $\pm$ 6.3 years). 
    % This dataset is manually pixel-wisely annotated~\cite{shattuck2008construction} by expert annotators. 
    The scans were acquired with a spatial resolution of 0.86 $\times$ 1.5 $\times$ 0.86 mm$^3$. Here, we conduct experiments on the subset of the hippocampus in LPBA40.
.
\end{itemize}

\subsection{Implementation details and evaluation metrics}
% based on Boxinst, following..., we set training: lr, epoch, decay....
% our models are trained with gpus , Pytorch
The proposed framework with geometric prior and contrastive similarity can be easily incorporated with any weakly-supervised segmentation models with bounding box annotations. To verify the robustness of our method, we conduct experiments with two models: Ai+L~\cite{chu2021improving} and BoxInst~\cite{tian2021boxinst}. Here, we take the latest BoxInst~\cite{tian2021boxinst} as our baseline, and experiments are conducted based on this model unless otherwise specified.
The training setting is mostly based on BoxInst's training settings: The basic learning rate is 0.01 with weight decay 1e-4, and a MultiStepLR scheduler with warmup is adopted. Our framework is trained on GeForce RTX 3090 GPU. During the inference stage, we set the threshold of the completeness head to 0.6 and the threshold of the class head to 0.5 empirically. We randomly select a training sample as the template for each specific dataset unless otherwise specified. We evaluate our results by two widely adopted metrics: the Dice score (DSC) in percentages and the Hausdorff Distance (95\%). 1) DSC score is calculated as the overlap area of two masks divided by their summation. A higher DSC score corresponds to better overlap with GT. 2) The Hausdorff Distance mainly measures the boundary distance between the segmentation result and the pixel-wise segmentation masks. Better segmentation results are of a smaller value than inferior results.

\textbf{Pre-processing \& Post-processing} Following nnUNet~\cite{isensee2021nnu}, the pre-processing includes downsampling, patching, and data augmentation. Here, we downsample the data to reduce memory use and ensure the existence of complete instances inside one patch. Then in the post-processing stage, the pipeline contains resampling, patching, and patch-NMS (Non-Maximum Suppression between patches). We first adjust the spacing and patch the data to the same size as training, with a certain step size. Then we predict a segmentation mask for each patch and return all the predictions to the original space. Since there are overlapping areas between patches, we use patch-NMS in these areas to eliminate the duplicates. 
% More technical details can be found in nnUNet~\cite{isensee2021nnu}.

\textbf{Bounding box annotation} We conduct experiments on LiTS, KiTS, and LPBA40 datasets. All these three datasets have pixel-wise segmentation annotations. We {utilize} the corresponding pixel-wise annotations to obtain the corresponding bounding-box annotations. In the training stage, only bounding-box annotations are included. During the inference stage, we evaluate the performance by pixel-wise annotations. 


\subsection{Results}

\textbf{Quantitative Results.} We report the quantitative results of three datasets (LiTS17, KiTS21, and LPBA40) in Tab.~\ref{tab:main_res}. 
Our method aims to integrate the geometric prior and contrastive similarity to give better supervision in the training of the weakly-supervised segmentation framework. Compared with BoxInst~\cite{tian2021boxinst}, which is the baseline of our method, the segmentation performance of our method is largely improved over all three datasets. This is because the geometric prior can supervise the learning of both outer shape and the inner structure, and the contrastive similarity better distinguishes organ and non-organ pixels in the embedding space. Similarly, ours outperforms the most recent two weakly-supervised methods~\cite{hu2021semi, Dolz2020} supervised by bounding-box annotations, which are based on the Multiple Instance Learning (\emph{i.e.}, MIL). The reason behind this is that MIL mainly focuses on the boundary regression of the proposal, but additionally, we learn the internal details of organs from the geometric prior. We also evaluate the upper bound of our method in which we supervise the framework training with ground truth. 

\textbf{Qualitative Results.} We present the qualitative comparison with two state-of-the-art weakly-supervised segmentation methods in Fig~\ref{fig:main_res}. Compared with BoxInst~\cite{tian2021boxinst}, which is the baseline of our framework, we well preserve the proposal's inner structure detail and outer shape. By comparing Column.\#4 and Column.\#7, the segmentation accuracy is largely improved compared to the baseline in Fig.~\ref{fig:main_res}. This is because the proposed geometric prior and the contrastive similarity help better segment organs. Additionally, the quality of our result is much better than other state-of-the-art methods, especially in terms of internal details. Their methods are based on Multiple Instance Learning (\emph{i.e.}, MIL, GMIL), which mainly focuses on the outer shape of the proposal ignoring the hollows inside the organs. In contrast to their methods, we learn the inner structure and geometric details from the given template organ along with the outer shape that boosts the training of the mask head.






\vspace{-0.1cm}
\subsection{Ablation Study}
In this subsection, we first present the component-wise analysis of our framework and then discuss the effectiveness of the proposed geometric prior and contrastive similarity. 

% todo
\begin{figure*}[ht]
    \setlength\tabcolsep{1.1pt}
    \centering
    \begin{tabularx}{\textwidth}{ccccccccc}
    &&\text{Input} &\text{GT}& \text{Fully} & \text{BoxInst} & \text{MIL} & \text{GMIL} & \text{Ours} \\
    
    \raisebox{0.65\height}{\rotatebox{90}{\text{Kidney}}}&
    \raisebox{0.32\height}{\rotatebox{90}{\text{Surface X}}}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_kits/input_x.jpg}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_kits/gt_x.jpg}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_kits/fully_x.jpg}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_kits/boxinst_x.jpg}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_kits/mil_x.jpg}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_kits/gmil_x.jpg}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_kits/ours_x.jpg}\\
    
    \raisebox{0.65\height}{\rotatebox{90}{\text{Kidney}}}&
    \raisebox{0.32\height}{\rotatebox{90}{\text{Surface Y}}}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_kits/input_y.jpg}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_kits/gt_y.jpg}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_kits/fully_y.jpg}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_kits/boxinst_y.jpg}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_kits/mil_y.jpg}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_kits/gmil_y.jpg}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_kits/ours_y.jpg}\\
    
    \raisebox{0.65\height}{\rotatebox{90}{\text{Kidney}}}&
    \raisebox{0.32\height}{\rotatebox{90}{\text{Surface Z}}}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_kits/input_z.jpg}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_kits/gt_z.jpg}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_kits/fully_z.jpg}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_kits/boxinst_z.jpg}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_kits/mil_z.jpg}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_kits/gmil_z.jpg}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_kits/ours_z.jpg}\\
    
    \raisebox{1.1\height}{\rotatebox{90}{\text{Liver}}}&
    \raisebox{0.32\height}{\rotatebox{90}{\text{Surface X}}}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_lits/input_x.jpg}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_lits/gt_x.jpg}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_lits/fully_x.jpg}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_lits/boxinst_x.jpg}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_lits/mil_x.jpg}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_lits/gmil_x.jpg}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_lits/ours_x.jpg}\\
    
    \raisebox{1.1\height}{\rotatebox{90}{\text{Liver}}}&
    \raisebox{0.32\height}{\rotatebox{90}{\text{Surface Y}}}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_lits/input_y.jpg}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_lits/gt_y.jpg}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_lits/fully_y.jpg}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_lits/boxinst_y.jpg}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_lits/mil_y.jpg}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_lits/gmil_y.jpg}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_lits/ours_y.jpg}\\
    
    \raisebox{1.1\height}{\rotatebox{90}{\text{Liver}}}&
    \raisebox{0.32\height}{\rotatebox{90}{\text{Surface Z}}}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_lits/input_z.jpg}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_lits/gt_z.jpg}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_lits/fully_z.jpg}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_lits/boxinst_z.jpg}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_lits/mil_z.jpg}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_lits/gmil_z.jpg}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_lits/ours_z.jpg}\\
    
    \raisebox{0.1\height}{\rotatebox{90}{\text{Hippocampus}}}&
    \raisebox{0.32\height}{\rotatebox{90}{\text{Surface X}}}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_lpba/input_x.jpg}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_lpba/lpba_gt_x.jpg}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_lpba/lpba_fully_x.jpg}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_lpba/boxinst_x.jpg}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_lpba/mil_x.jpg}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_lpba/gmil_x.jpg}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_lpba/ours_x.jpg}\\
    
    \raisebox{0.1\height}{\rotatebox{90}{\text{Hippocampus}}}&
    \raisebox{0.32\height}{\rotatebox{90}{\text{Surface Y}}}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_lpba/input_y.jpg}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_lpba/lpba_gt_y.jpg}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_lpba/lpba_fully_y.jpg}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_lpba/boxinst_y.jpg}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_lpba/mil_y.jpg}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_lpba/gmil_y.jpg}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_lpba/ours_y.jpg}\\
    
    \raisebox{0.1\height}{\rotatebox{90}{\text{Hippocampus}}}&
    \raisebox{0.32\height}{\rotatebox{90}{\text{Surface Z}}}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_lpba/input_z.jpg}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_lpba/lpba_gt_z.jpg}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_lpba/lpba_fully_z.jpg}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_lpba/boxinst_z.jpg}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_lpba/mil_z.jpg}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_lpba/gmil_z.jpg}&
    \includegraphics[width=0.13\linewidth]{figs/main_res_lpba/ours_z.jpg}\\
    
    
    
    \end{tabularx}
    \caption{\small{Qualitative results of our framework over three datasets. 
    As shown in the figure, four colors exist in the segmentation results. {\em red} indicates ground-truth. {\em green} indicates correct predictions. {\em blue} indicates predictions where should have been predicted. {\em yellow} indicates wrongly-predicted pixels. 
    Our framework is built on BoxInst~\cite{tian2021boxinst} which is the baseline method. We then compare several methods, including fully-supervised results, the proposed method and demonstrate the high quality of the proposal.}}
    \label{fig:main_res}
\end{figure*}


\subsubsection{Robustness}
In this subsection, we mainly discuss the robustness of the proposed weakly-supervised segmentation framework. Our framework is built on BoxInst~\cite{tian2021boxinst}, which is composed of Backbone and FPN. We analyze the impact of the backbone on the weakly-supervised segmentation performance. As shown in Tab.~\ref{tab:robuseness}, our method is robust to other backbones ({\em i.e.}, ResNet~\cite{he2016deep} and U-Net~\cite{ronneberger2015u}). Furthermore, we verify the generality of the proposed framework by extending to other weakly-supervised segmentation models. Following Chu \emph{et al.}~\cite{chu2021improving}, we use the Ai+L~\cite{chu2021improving} model with a ResNet50~\cite{he2016deep} backbone that is widely used in both non-medical~\cite{lateef2019survey} and medical~\cite{anderson2021automated} segmentation tasks. We concatenate the geometric prior branch and contrastive similarity branch after the decoder. As shown in Tab.~\ref{tab:robuseness}, the baseline model obtains 67.2\% in the KiTS dataset. The segmentation performance is largely improved by 4.9\% after adding the proposed geometric prior and contrastive similarity losses. 

\begin{table}[t!]
\small
\centering
\caption{\small{Robustness analysis. We measure the corresponding dice score on the KiTS21 dataset. We implement the 3D version of BoxInst~\cite{tian2021boxinst} based on its 2D version public code.}}
\renewcommand\arraystretch{1.4}
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
\scalebox{0.98}{
	\begin{tabular}{cP{2.1cm}P{2.1cm}cc}
		\specialrule{.8pt}{0pt}{2pt}
		\multirow{2}{*}{\#}& \multirow{2}{*}{Backbone} & \multirow{2}{*}{Model} & Without & With\\
% 		\cline{4-5}
		& & & Our Loss&Our Loss\\
		\specialrule{.4pt}{2pt}{0pt}
% 		\rowcolor[gray]{.9}
		1&ResNet~\cite{he2016deep}&BoxInst 3D~\cite{tian2021boxinst}& 47.8 & \textbf{77.1}\\
		2&UNet~\cite{ronneberger2015u}&BoxInst 3D~\cite{tian2021boxinst}& 49.1& \textbf{80.2}\\
		3&ResNet~\cite{he2016deep}&Ai+L~\cite{chu2021improving}&67.2 & \textbf{72.1}\\
		
% 		1 &  & \checkmark &  & \checkmark &  &  67.2\\
% 		2 &  & \checkmark &  & \checkmark & \checkmark &  76.9\\
% 		3 & \checkmark &  & \checkmark &  & \checkmark &  67.2\\
% 		4 & \checkmark &  &  & \checkmark & \checkmark &  76.9\\
% 		5$^\ddagger$ & \checkmark &  & \checkmark &  &  &  91.7\\
% 		6$^\ddagger$ & \checkmark &  &  & \checkmark &  &  96.0\\
		\specialrule{.8pt}{0pt}{2pt}
	\end{tabular}
}
\label{tab:robuseness}
\vspace{-0.6cm}
\end{table}

% 3:add another

% % ***Additionally, we also verify the effectiveness of the proposed geometric prior and contrastive similarity in supervised segmentation schemes. 

% \begin{table}[!b]
% 	\small
% 	\centering
% 	\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
%     \resizebox{1.\linewidth}{!}{
%         \begin{center}
%     		\begin{tabular}{c|P{4.7cm}|c|c}
%     			\toprule[1.07pt]
%     			\# & Backbone Setting & Weakly? &Dice Score \\
%     			\midrule[1.07pt]
%     			1 & 3D ResNet~\cite{he2016deep} &\CheckmarkBold& -  \\
%     			2& 3D ResNet~\cite{he2016deep}&\XSolidBrush & 91.7  \\
%     			3& UNet~\cite{ronneberger2015u} &\CheckmarkBold & 79.9 \\
%     			4& UNet~\cite{ronneberger2015u} &\XSolidBrush & 96.0 \\

%     			\bottomrule[1.07pt]
%     		\end{tabular}
%     	\end{center} 
% 	}
% 	\caption{{Backbone Analysis. $\dagger$: we measure the corresponding dice score on the KiTS21 dataset. $\text{Weakly?}$ indicates whether the method is weakly-supervised or fully-supervised.}}
% 	\label{tab:backbone}
% 	\normalsize
% \end{table}



\subsubsection{Geometric prior}
% \textbf{Analysis of the template selection}
In the proposed geometric prior, we minimize the Chamfer Distance between the template organ and the proposal in the point cloud embedding space. The point cloud representation is much more flexible than the volume representation. This is because the volume representation is constrained by the uniform voxel grids. The representative point of each grid is fixed to the center of each corresponding grid. In contrast, there is no such constraint in the point cloud representation. The coordinates of points are much more precise and flexible elastic ({\em i.e.}, \{0.17, 0.18, ...\} \emph{v.s.} \{1.00, 2.00, ...\}). This helps the point cloud representation to better describe delicate and complex structures than the conventionally-used volume representation. 
Thus, to validate this point, we conduct an ablation of registration and optimization with the volume representation. More specifically, we first register the organ by the widely-used SimpleITK~\cite{lowekamp2013design}. Here, the registration settings are set as follows: Mean Square metric, random sampling strategy with a percentage of 0.01, shrink factors $[4, 2, 1]$, smoothing sigmas $[2, 1, 0]$, and 100 iterations.
After the registration, we employ the Dice loss to optimize the distance between the segmentation result and the geometric prior. As shown in Fig.~\ref{fig:represent}, the result shows that the point cloud representation can handle more complex architectures and precise geometric shapes, by improving 4.3\% in the Dice Score Coefficient.

\begin{table}[!b]
	\small
	\vspace{-0.6cm}
	\centering
	\caption{{Analysis of geometric prior. $\dagger$ indicates the inner structure of the template.}}
	\renewcommand\arraystretch{1.4}
	\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
    \resizebox{0.97\linewidth}{!}{
    		\begin{tabular}{cP{4.7cm}P{2.3cm}}
    			\specialrule{.8pt}{0pt}{2pt}
    			\multirow{2}{*}{\#}& \multirow{2}{*}{Ablation Setting} & DSC on \\
		        & &  KiTS \\
    			\specialrule{.4pt}{2pt}{0pt}
    			1 & {w/o Completeness Head} &\multicolumn{1}{c}{79.1}\\
    			2 & w/o $\text{Internal Details}^{\dagger}$ &\multicolumn{1}{c}{76.3} \\
    			\rowcolor[gray]{.9}
    			3 & Baseline & 80.2 \\
    			\specialrule{.8pt}{0pt}{2pt}
    		\end{tabular}
    % 	\end{center} 
	}
	\label{tab:cpl_internal}
	\normalsize
\end{table}
\newcommand{\setgray}{\cellcolor[gray]{.9}}
\begin{table}[!b]
	\small
	\centering
	\vspace{-0.3cm}
	\caption{{Analysis of the contrastive head. $\dagger$: C stands for the contrastive similarity, S indicates the SSIM similarity and G stands for the grayscale similarity. The inference speed indicates the total time of 1000 runs.}}
	\renewcommand\arraystretch{1.4}
	\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
    \resizebox{1.\linewidth}{!}{
        % \begin{center}
    		\begin{tabular}{cP{3.5cm}cccc}
    			\specialrule{.8pt}{0pt}{2pt}
    % 			
    			\multirow{2}{*}{\#} & \multirow{2}{*}{Component Setting}  & Embedding & Embedding & Inference & DSC (\%) \\
    			&  & Dimension &Space$^\dagger$ & Speed & on KiTS\\
                \specialrule{.4pt}{2pt}{0pt}
    			 1 & \multirow{4}{*}{Contrastive Head} &  8 &  C &  3s &  78.4\\
    			2 & &16 & C & 5s & 79.1\\
    			 3 & & 32 &  C &  8s &  80.2\\
    			4 & &64 & C & 15s & 80.4\\
    			\specialrule{.4pt}{2pt}{0pt}
    			 5 & \multirow{3}{*}{Similarity Metrics} & 32&  C &  8s &  80.2\\
    			6 & &32 & G & 8s & 73.4\\
    			 7 & & 32 &  S &  12s &  47.2\\
                % \hline
    			\specialrule{.8pt}{0pt}{2pt}
    		\end{tabular}
	}
	\label{tab:cpl_internal}
	\normalsize
\end{table}

\textbf{Internal details}
We further analyze the impact of the template from the perspective of outer shape and inner structures, respectively. The experiments in this subsection are organized as follows: We first fulfill the inner structure of the template and only retain the outer shape. Then we train the mask head with the deformed template. Normally, there exists intra-organ variabilities, \emph{i.e.}, as shown in Fig.~\ref{fig:internal}, especially meticulous architectures inside the kidney. And the segmentation performance drastically degrades (3.9\%) for the lack of internal prior. 

% todo
\begin{figure}[!tb]
    \setlength\tabcolsep{1.6pt}
    \centering
    \small
    \begin{tabularx}{\textwidth}{cccc}
    % \raisebox{0.1\height}{\rotatebox{90}{\text{Ground Truth}}}&
    % \includegraphics[width=0.92\linewidth]{figs/input_boundary.png}\\
    
    \raisebox{1.2\height}{\rotatebox{90}{\text{Input}}}&
    \includegraphics[width=0.3\linewidth]{figs/pc_volume/input_x.jpg}&
    \includegraphics[width=0.3\linewidth]{figs/pc_volume/input_y.jpg}&
    \includegraphics[width=0.3\linewidth]{figs/pc_volume/input_z.jpg}\\
    
    \raisebox{0.8\height}{\rotatebox{90}{\text{volume}}}&
    \includegraphics[width=0.3\linewidth]{figs/pc_volume/volume_x.jpg}&
    \includegraphics[width=0.3\linewidth]{figs/pc_volume/volume_y.jpg}&
    \includegraphics[width=0.3\linewidth]{figs/pc_volume/volume_z.jpg}\\
    
    \raisebox{0.35\height}{\rotatebox{90}{\text{point cloud}}}&
    \includegraphics[width=0.3\linewidth]{figs/pc_volume/pc_x.jpg}&
    \includegraphics[width=0.3\linewidth]{figs/pc_volume/pc_y.jpg}&
    \includegraphics[width=0.3\linewidth]{figs/pc_volume/pc_z.jpg}\\

    \end{tabularx}
    \caption{\small{Volume {\em v.s.} Point cloud. We optimize the learning of the geometric shape in the form of volume representation by Dice Loss. As shown in the figure, the proposed point cloud representation largely improves the segmentation result.} }
    \label{fig:represent}
\end{figure}
\begin{figure}[!tb]
    \setlength\tabcolsep{1.6pt}
    \centering
    \small
    \begin{tabularx}{\textwidth}{cccc}
    % \raisebox{0.1\height}{\rotatebox{90}{\text{Ground Truth}}}&
    % \includegraphics[width=0.92\linewidth]{figs/input_boundary.png}\\
    
    \raisebox{1.2\height}{\rotatebox{90}{\text{Input}}}&
    \includegraphics[width=0.3\linewidth]{figs/internal/input_case1.jpg}&
    \includegraphics[width=0.3\linewidth]{figs/internal/input_case2.jpg}&
    \includegraphics[width=0.3\linewidth]{figs/internal/input_case3.jpg}\\
    
    \raisebox{0.38\height}{\rotatebox{90}{\text{w/o internal}}}&
    \includegraphics[width=0.3\linewidth]{figs/internal/wo_case1.jpg}&
    \includegraphics[width=0.3\linewidth]{figs/internal/wo_case2.jpg}&
    \includegraphics[width=0.3\linewidth]{figs/internal/wo_case3.jpg}\\
    
    \raisebox{0.38\height}{\rotatebox{90}{\text{w internal}}}&
    \includegraphics[width=0.3\linewidth]{figs/internal/w_case1.jpg}&
    \includegraphics[width=0.3\linewidth]{figs/internal/w_case2.jpg}&
    \includegraphics[width=0.3\linewidth]{figs/internal/w_case3.jpg}\\

    \end{tabularx}
    \caption{\small{Internal details. To verify the effectiveness of the internal details of the template, we erase the intra-organ variabilities by fulfilling the template organ. As shown in the figure, the segmentation performance drastically degrades especially for organs with delicate and complex structures. Figures from left to right are more and more delicate and complex.} }
    \label{fig:internal}
    \vspace{-0.6cm}
\end{figure}
% todo
%  \begin{figure}[!tb]
%     \setlength\tabcolsep{1.6pt}
%     \centering
%     \small
%     \begin{tabularx}{\textwidth}{cccc}
%     % \raisebox{0.1\height}{\rotatebox{90}{\text{Ground Truth}}}&
%     % \includegraphics[width=0.92\linewidth]{figs/input_boundary.png}\\
    
%     \raisebox{0.38\height}{\rotatebox{90}{\text{w/o internal}}}&
%     \includegraphics[width=0.3\linewidth]{figs/main_res_kits/fully_x.jpg}&
%     \includegraphics[width=0.3\linewidth]{figs/main_res_kits/fully_x.jpg}&
%     \includegraphics[width=0.3\linewidth]{figs/main_res_kits/fully_x.jpg}\\
    
%     \raisebox{0.32\height}{\rotatebox{90}{\text{w/o boundary}}}&
%     \includegraphics[width=0.3\linewidth]{figs/main_res_kits/fully_x.jpg}&
%     \includegraphics[width=0.3\linewidth]{figs/main_res_kits/fully_x.jpg}&
%     \includegraphics[width=0.3\linewidth]{figs/main_res_kits/fully_x.jpg}\\
    
%     \raisebox{0.65\height}{\rotatebox{90}{\text{baseline}}}&
%     \includegraphics[width=0.3\linewidth]{figs/main_res_kits/fully_x.jpg}&
%     \includegraphics[width=0.3\linewidth]{figs/main_res_kits/fully_x.jpg}&
%     \includegraphics[width=0.3\linewidth]{figs/main_res_kits/fully_x.jpg}\\

%     \end{tabularx}
%     \caption{\small{Internal details and geometric shape. 1) We erase the internal detail of the template and compare the result segmentation with the baseline as in Row \# 1. 2) We then deform the template to other geometric shape to evaluate the effectiveness of the geometric prior as in Row \#2.} }
%     \label{fig:internal}
% \end{figure}

%  \begin{figure}[!tb]
%     \setlength\tabcolsep{1.6pt}
%     \centering
%     \small
%     \begin{tabularx}{\textwidth}{cccccc}
%     &\text{Template Geo.} & \text{Input Image} & \text{Optim. Result}\\
    
    
%     \raisebox{0.75\height}{\rotatebox{90}{\text{Kidney}}}&
%     \includegraphics[width=0.31\linewidth]{figs/kidney_template.png}&
%     \includegraphics[width=0.31\linewidth]{figs/1res1.png}&
%     \includegraphics[width=0.31\linewidth]{figs/1res1.png}\\
    
%     \raisebox{1.1\height}{\rotatebox{90}{\text{Cube}}}&
%     \includegraphics[width=0.31\linewidth]{figs/template_cube.png}&
%     \includegraphics[width=0.31\linewidth]{figs/1res1.png}&
%     \includegraphics[width=0.31\linewidth]{figs/1res1.png}\\


%     \end{tabularx}
%     \caption{\small{Analysis of template boundary. We deform the boundary of the template. And we train the segmentation framework using the deformed template. Obviously, the generated proposal is largely influenced by the template boundary.} }
%     \label{fig:template_shape}
% \end{figure}


%  \begin{figure}[!tb]
%     \setlength\tabcolsep{1.6pt}
%     \centering
%     \small
%     \begin{tabularx}{\textwidth}{cccc}
   
    
    
%     \includegraphics[width=0.23\linewidth]{figs/1res1.png}&
%     \includegraphics[width=0.23\linewidth]{figs/1res2.png}&
%     \includegraphics[width=0.23\linewidth]{figs/1res3.png}&
%     \includegraphics[width=0.23\linewidth]{figs/1res4.png}\\
    
%     % \raisebox{\height}{\rotatebox{90}{\text{Fine}}}&
%     % \includegraphics[width=0.23\linewidth]{figs/2res1.png}&
%     % \includegraphics[width=0.23\linewidth]{figs/2res2.png}&
%     % \includegraphics[width=0.23\linewidth]{figs/2res3.png}&
%     % \includegraphics[width=0.23\linewidth]{figs/2res4.png}\\

%     \end{tabularx}
%     \caption{\small{Template optimization. We present the learning process between the proposal and the template. The matching is conducted in a global-to-local fashion.} }
%     \label{fig:evo}
% \end{figure}

%  \begin{figure}[!tb]
%     \setlength\tabcolsep{1.6pt}
%     \centering
%     \small
%     % \includegraphics[width=0.97\linewidth]{figs/withoutinternal.png}\\
%     \includegraphics[width=0.99\linewidth]{figs/cpl.png}   \\

%     \caption{\small{Incomplete Kidney due to the pre-processing procedure. We alleviate this by leveraging the completeness head.} }
%     \label{fig:organ_hollow}
% \end{figure}

% \textbf{Geometry shape} Then, we further analyze the impact of the template on the geometry regression of the proposal. The template introduce geometric shape into  the training of the weakly-supervised segmentation framework. We then deform the boundary shape of the template via randomly generated affine matrix. As shown in Fig.~\ref{fig:template_shape}, we supervise the training of the mask head by different variations of the template. As the boundary shape of the template varies, the generated proposal have different boundary shapes accordingly. This is because the Chamfer Distance encourages the overall structure of the template and the generated proposal similar. And we can notice that the generated proposal is not exactly the same as the deformed template, the reason behind this is that the contrastive similarity can make the boundary of the generated proposal fit the organ shape better by aligning the positive locations in the embedding space, which plays a confrontational role.

\textbf{Analysis of the completeness head}
As discussed in Sec.~\ref{sec:overall}, following nnUNet~\cite{isensee2021nnu}, for an input image, we first partition it into patches and sequentially process these patches. However, during the partitioning, organs may not be complete, which may cause the failure of the learning from the template. Thus, to ensure the success of learning from the template, the proposed completeness head detects whether the proposal in the sampled patch is complete. Only complete proposals are further processed. As shown in Tab.~\ref{tab:cpl_internal}, if we remove the completeness head, the performance degrades by 1.1\% compared with our framework. 
% This is because input image patches containing only part of the organ will be handled as a complete organ to fit the template during the learning process, resulting in a significant performance drop in the segmentation result.



\subsubsection{Architectures of contrastive head}
We conduct experiments on the design of the proposed contrastive head in this subsection. Following previous works~\cite{chen2020simple, hu2021semi}, the contrastive head is composed of a two-layer point-wise convolution that helps distinguish organ tissues from non-organ tissues. To further analyze the structure of the contrastive head, we conduct ablation experiments on the dimension of the embedding space. As shown in Tab.~\ref{tab:cpl_internal}, we evaluate both the performance and the efficiency of different embedding dimension that by considering the trade-off between efficiency and performance, we empirically set the embedding dimension to 32.

\textbf{Contrastive similarity}
 We propose the contrastive similarity in the embedding space. To compare the embedding space with the commonly used gray space, we select the following two similarity metrics: \textit{MSE} and \textit{SSIM}~\cite{wang2004image}. Both \textit{MSE} and \textit{SSIM} are calculated on gray values since medical images are in grayscale. {As shown in Tab.~\ref{tab:cpl_internal}, the \textit{MSE} metric fails to distinguish low-contrast tissues,} and the \textit{SSIM} metric is inferior to the contrastive similarity in terms of both segmentation performance and evaluation efficiency.



==> chap/intro.tex <==
\vspace{-0.2cm}
\section{Introduction}
\label{sec:intro}
\IEEEPARstart{S}{egmentation} is of fundamental importance for the understanding and interpretation of medical images, as it is essential for the diagnostic, treatment, and follow-up rehabilitation of various diseases. This task has been widely studied with the recent advent of deep convolutional neural networks (CNNs) ~\cite{ronneberger2015u, isensee2021nnu}. Nevertheless, there exists the main limitation that their methods require a large number of training images with pixel-wise annotations. The extremely high cost of collecting and annotating these training images largely hampers the performance and limits the scalability of deep CNNs in the medical domain. A popular paradigm to alleviate the need for pixel-wise annotations is the weakly-supervised segmentation with bounding-box annotations~\cite{pathak2015constrained,jia2017constrained,kervadec2019constrained,bateson2019constrained, tian2021boxinst}. They employ bounding-box annotations to generate { proposals}, which are {fake} labels and thereby mimic full supervision.
% ,. researchers have looked at training these instance segmentation models
% using weak annotations, This largely 
% the need of annotated datasets 



 \begin{figure}[!tb]
    \setlength\tabcolsep{1.6pt}
    \centering
    \small
    \includegraphics[width=\linewidth]{figs/intro.pdf}
    \caption{\small{The illustration of the proposed weakly-supervised segmentation framework. As shown in the figure, we propose geometric prior and contrastive similarity for weakly-supervised segmentation. The top row indicates the geometric prior of our method. We first convert the conventionally-used volume representation to point cloud representation and register the template organ to the predicted organ. Then we minimize their Chamfer Distance. The bottom row explains the core idea of the proposed contrastive similarity. By dividing pixels into positive and negative pixels, we encourage organ pixels to gather around in the embedding space to better segment the low-contrast organ.}}
    \label{fig:intro}
    \vspace{-0.3cm}
\end{figure}

%\newcommand{\qone}{{geometric discontinuty}}
\newcommand{\qone}{{complex shapes}}
\newcommand{\qtwo}{{imaging artifacts}}
Nevertheless, despite the good performances achieved by these works in certain practical scenarios, their applicability might be limited for two reasons: 1) {\em \qone}: Some organs have delicate structures {\em, i.e.}, intra-kidney variabilities, which are difficult to be precisely segmented without pixel-wise supervision;
2) {\em \qtwo}: as discussed in previous works~\cite{budrys2018artifacts, boas2012ct,sarkar2018subjective}, various medical imaging artifacts caused by technical or physical problems make low-contrast tissues and non-homogenous textures hard to distinguish, especially in the conventionally widely-used gray space. 
The \qone\ and \qtwo\ largely limit the applicability of the weakly-supervised segmentation models in many scenarios, especially when segmenting complex structures. 
        


% A few recent work have been proposed to address the above-mentioned issues~\cite{huang2021medical, wang2021bounding, hsu2019weakly}. Huang {\em et al.}~\cite{huang2021medical} propose to calculate the probabilistic organ distribution of a given pixel-wise dataset and incorporate the calculated prior into the training loss. Despite the good performance achieved by the proposed atlas prior, the generated proposal lacks of 3d consistency because the calculated prior is applied in 2d slices and the correlation between 2D slices is ignore. This largely degrades the segmentation quality. Furthermore, it requires pixel-wise annotations  of the dataset to calculate the probabilistic  distribution which is infeasible in weakly-supervised scenarios. (move into related work, 2d -> 3D volume -> point cloud ads)
% ads in intro, differs in related work
% 1: 2d->3d
% 2: fine level geo detail (coarse)

% to address the first
% .
% .second....but their problem

% unlike xxxx, we propose pc, ads
% different from we xxx, contr., ads (below para)

To conquer the challenge of \qone\, we propose to learn the geometric prior of the organ by a standard organ template. Instead of using volume representation, we first leverage the gridding reverse~\cite{xie2020grnet} to convert the segmentation result from volume representation to point cloud representation and then compare it with the template in the point cloud space. The basic unit in point cloud representation is much more fine-grained and flexible than the volume representation ({\em, i.e.}, flexible point {\em v.s.} uniform voxel grids), which helps better describe delicate geometric structures. On the other hand, unlike the conventionally-used gray space~\cite{budrys2018artifacts}, we leverage the contrastive learning~\cite{chaitanya2020contrastive} to encode the pixels to high-dimensional embedding space and encourage pixels of the same labels to gather around. This helps alleviate the \qtwo\ for richer expressivity in the embedding space compared to the gray space.

% This learning process is conducted in the form of point cloud. 

% Our method is inspired by the recent progress in point cloud segmentation~\cite{xie2020grnet} and contrastive learning~\cite{chaitanya2020contrastive}, respectively. 
% Xie {\em et al.} propose the gridding reverse to build the conversion bridge between point cloud and voxel. Comparing with voxel representation, it's easier to capture the spatial relationship in point cloud representation which can help better learn the geometry of the prior. 
% Then from the perspective of contrastive learning, Krishna {\em et al.}~\cite{chaitanya2020contrastive} proposes to force pixels with the same label ({\em i.e.}, foreground or background) to gather around in the embedding space. However, it requires pixel-wise annotations which is infeasible in the weakly-supervised segmentation. 


In this paper, we present a novel weakly-supervised segmentation framework, which makes the earliest effort to incorporate geometric prior and contrastive similarity. And the framework is general as well that can be easily applied to improve multiple weakly-supervised segmentation models with bounding-box annotations, \emph{i.e.}, Ai+L~\cite{chu2021improving}, BoxInst~\cite{tian2021boxinst}. By learning geometry prior from the given template and distinguishing low-contrast tissues by the contrastive similarity, our method can generate high-quality results with bounding box supervision only. 

Our method consists of two major components. In the geometric prior component, the shapes of proposals are constrained by a given template represented by point cloud. Both the external boundaries and internal structures of the proposal will be optimized by minimizing the distance according to a given template. The second component is the contrastive similarity, addressing the issues raised by medical imaging artifacts. By pre-training a contrastive head, we successfully learn the difference between organ pixels and non-organ pixels. This component can better distinguish low-contrast tissues and non-homogenous texture than conventionally widely-used gray space. Through extensive experiments, we demonstrate that our method can generate a high-quality segments, along with delicate internal details and accurate boundaries. We show that our method outperforms other bounding-box weakly-supervised methods ~\cite{tian2021boxinst, kervadec2019constrained} under similar settings. We also conduct extensive experiments to verify the effectiveness of components in our method.

In summary, our major contributions are three folds.
\begin{itemize}
    \item We propose a simple yet effective weakly-supervised segmentation framework with bounding-box annotations, which can be easily applied to many weakly-supervised segmentation models and improve their performances.
    \item We propose the geometric prior in point cloud representation to better guide the learning of shapes, especially for those organs with complex structures.
    \item The proposed contrastive similarity makes up for the poor representation of the conventional gray space and thus can better distinguish tissues with medical imaging artifacts.
\end{itemize}
Our code and data will be made publicly available for further research.

% The remainder of this paper is organized as follows.
% Section II introduces related work. The proposed geometric prior
% and contrastive similarity are described in Section III.
% Subsequently, Section IV discusses experiments and results,
% and finally Section V concludes the paper.

==> chap/method.tex <==
\section{Method}
\label{sec:method}
% \IEEEPARstart{I}{n} this section, we first briefly introduce the overall architecture of the proposed framework. Then we elaborate the technical details of the propsoed arning loss and shape loss.





\subsection{Overall framework}
\label{sec:overall}
\newcommand{\R}{\mathbb{R}}
\newcommand{\qihua}[1]{\textcolor{blue}{#1}}
% Given an input image $I \in \RR^{S \times H \times W}$, the goal of our weakly-supervised framework is to obtain the pixel-level segmentation mask. We first partition the input image into patches $p \in \R^{S \times H \times W}$ and encode the patches into a  {sequence} by a ConvNet encoder $E$. Similar to ~\cite{ronneberger2015u}

{Given an input image $I \in \R^{S \times H \times W}$ ($S$ indicates the slice number, $H$ indicates height and $W$ represents width) and its corresponding bounding-box annotation $\mathbb{B}^{1\times 6}$ (constrained by its upper left coordinates and bottom right coordinates), our weakly-supervised framework $\mathbf{F}(\cdot)$ obtains the pixel-wise segmentation mask $\mathcal{M}=\mathbf{F}(I)$ and the training goal is to minimize the loss function $L_\text{frame}$:
\begin{equation}
\begin{aligned}
\label{eq:overall_formu}
  \min_{\mathbf{F}}{L_\text{frame}(I, \mathbb{B}, \mathbf{F})}
\end{aligned}
\end{equation}

\textbf{Pipeline} Following nnUNet~\cite{isensee2021nnu}, we randomly sample an input patch $p \in \R^{S' \times H' \times W'}$ from the original input image and encode the patches by a ConvNet encoder $E$. Similar to ~\cite{ronneberger2015u}, we adopt a multi-layer ConvNet as the decoder $G$ to obtain the feature maps $P \in \R^{S' \times H' \times W'}$, where the decoder shares the same layer number as the encoder.} As shown in Fig.~\ref{fig:method}, the proposed geometric prior and contrastive learning are incorporated in the training of the \textit{mask head} to address the aforementioned \qone\ and \qtwo\ issues. The training loss $L_{\text{frame}}$ is composed of two components: $L_{\text{ori}}$ and $L_{\text{mask}}$ 
\begin{equation}
\label{eq:frame_onerall}
\begin{aligned}
    L_{\text{frame}} = L_{\text{ori}} + L_{\text{mask}}
\end{aligned}
\end{equation}
where $L_{\text{ori}}$ indicates the original training loss of a standard weakly-supervised framework ({\em i.e.}, $L_{fcos}$ in BoxInst~\cite{tian2021boxinst}) and $L_{\text{mask}}$ stands for the training loss of the mask head. In the following paragraphs, we mainly discuss the training of the mask head. The training of the mask head can be formulated as Eq.\eqref{eq:overall}. 
\begin{equation}
\label{eq:overall}
\begin{aligned}
    L_{\text{mask}} = L_{\text{geo}} + L_{\text{cons}}
\end{aligned}
\end{equation}
The mask head produce binary segmentation masks which is further optimized by our proposed geometric prior $L_{\text{geo}}$ and contrastive similarity $L_{\text{cons}}$.  More specifically, for geometric prior loss, we build a \textit{completeness head} to predict the completeness score for every proposal, indicating the conditional probability that the object is complete {inside the input}. Each complete proposal is converted into point cloud and registered with the point cloud of the template organ. The Chamfer Distance loss is applied to minimize their distance. In the aspect of the contrastive similarity loss, we build a \textit{contrastive head} to obtain the contrastive similarity by the feature maps that the contrastive head assigns positive and negative labels to each position in the feature maps. 
% Following \cite{tian2019fcos, tian2021boxinst}, locations on the feature maps $P_i$ are classified into positive and negative samples by whether they are associated with an instance (\emph{i.e.}, positive indicates high association). More specifically, there exists mapping between a location $(x,~y)$ on the feature maps and a pixel $(\lfloor \frac{r}{2} \rfloor~+xr, \lfloor \frac{r}{2} \rfloor~+yr)$ in the input image where $r$ indicates the down-sampling ratio. Mapped locations in the center region of the input image is considered to be positive samples, and vice versa. Here, following previous works~\cite{tian2019fcos, tian2021boxinst}, the center region is defined as $(C_x-\rho r, C_y-\rho r, C_x+\rho r, C_y +\rho r)$ where $(C_x, C_y)$ is the center of the bounding box and $\rho$ is a hyperparameter as in ~\cite{tian2019fcos}. Same as ~\cite{tian2020conditional}, we build \textit{classification}, \textit{center-ness}, \textit{box} and \textit{mask} heads for each location $P_i$. The \textit{classification head} is to predict the class of each location (\emph{i.e.}, instance classes or background). The \textit{box} heads is to predict the bounding box coordinates, while the \textit{center-ness} heads predict the IOU of the predicted bounding box with labels. The \textit{mask head} predicts the segmentation mask by the given $P$.
% More technical details (\emph{i.e.}, training and architectures) can be referred to ~\cite{tian2020conditional, tian2021boxinst}.
% \textbf{Completeness head} Except for the above-mentioned heads, we also build the \textit{completeness head} to predict the completeness score for every candidate box indicating the conditional probability that the object is complete, considering the patch partitioning may divide organs into separated components. More specifically, in the inference stage, the \textit{completeness head} predicts completeness score for each candidate bounding box. Only proposals of high completeness score can be further processed by mask head. 
% move to geo, loss merge into Lgeo, add head in method ()
% In general, the overall training scheme of our weakly-supervised framework is built on BoxInst~\cite{tian2021boxinst} and we mainly discuss the training of the \textit{mask head}. More specifically, the mask head produce binary segmentation masks which is further optimized by our proposed geometric prior $L_{\text{geo}}$ and contrastive similarity $L_{\text{cons}}$. More specifically, for the contrastive similarity loss, we build a \textit{contrastive head} to obtain the contrastive similarity by the feature maps that the contrastive head assign positive and negative labels to each position in the feature maps. In the aspect of geometric prior loss, we first convert the binary segmentation mask to point cloud by the gridding reverse function ~\cite{xie2020grnet}. To avoid mismatching, we perform point cloud registration between the converted point cloud and the given template organ point cloud. Then we apply the Chamfer Distance loss to optimize the distance between the proposal and the template. In the following paragraphs, we first briefly introduce the overall architecture of the proposed framework. Then we elaborate the technical details of the proposed components.
In the following paragraphs, we first introduce the geometric prior. Then we elaborate on the technical details of the proposed contrastive similarity.


% The training of our weakly-supervised framework is built on BoxInst~\cite{tian2021boxinst}, which is in an end-to-end fashion. Different from BoxInst, we propose the geometric prior $L_{\text{geo}}$ and contrastive similarity $L_{\text{cons}}$ to guide the training of the \textit{mask head}. More specifically, for each proposal of high confidence score and completeness score, the \textit{mask head} predicts a binary mask for the instance. And this binary segmentation mask is further optimized by $L_{\text{geo}}$ and $L_{\text{cons}}$. 


\vspace{-0.35cm}
\subsection{Geometric Prior}
% 先讲geo prior是什么，怎么优化,loss是什么
% 然后一段讲sparse reg
% 讲一下completeness head训练

% template shishenme
% In this section, we first introduce the concept of the geometric prior, then we discuss how the geometric prior incorporate the training of the \textit{mask head} and finally we present the sparse registration of our framework.
% for sec b&c:
% separate para:
% first pipeline (how, regis, motivation stress)
% why point cloud (2d why fail)

% then overall pipeline,
% finally detailed training  loss

The proposed geometric prior is applied in 3D point cloud space for two reasons: 1) we observe that 2D slices cannot well-preserve the geometric continuity of 3D organs. Thus, we learn the geometric shape of the organ in 3D embedding space. 2) The conventionally-used volume representation cannot handle the segmentation of meticulous structures. The expressivity of the volume representation is largely limited by the uniform voxel grids. Instead, we leverage gridding reverse~\cite{xie2020grnet} to process the segmentation of complex shapes in point cloud embedding space. 
% Furthermore, 



As shown in Fig.~\ref{fig:method}, we propose the geometric prior to better weakly supervise the training of the mask head. The geometric prior refers to the template organ's boundary shape and internal distribution. More specifically, we introduce gridding reverse~\cite{xie2020grnet} to building a bridge between the volume representation and point cloud representation conversion. This helps us to get rid of the representation constraint in the volume representation. After converting both template organ $\mathbb{T}$ and proposal $\mathbb{S}$ into the point cloud representation, we then register the template organ to the proposal by a widely-used ICP registration tool~\cite{Zhou2018}. We finally minimize the geometric prior loss of the Chamfer Distance between the template organ and the proposal in the point cloud embedding space. Below we first introduce the conversion and registration of point cloud and then the definition of geometric prior loss.

\textbf{Conversion \& Registration} To utilize the rich expressivity in
point cloud representation, we introduce the gridding reverse~\cite{xie2020grnet} to help the transition between the volume representation and the point cloud representation. For each voxel grid, the gridding reverse calculates the weighted sum of the eight vertices of the corresponding grid and assigns the weighted sum to coordinates of a new point. Unlike uniform voxel grids, the high flexibility of points' coordinates enable the point cloud representation to describe meticulous and complex architectures. This helps better learn the difficult intra-organ variabilities in the weakly-supervised segmentation. Furthermore, we propose the sparse registration, which is applied before calculating the Chamfer Distance between $\mathbb{S}$ and $\mathbb{T}$. Tiny rotation of the template greatly impacts the calculation of the Chamfer Distance, especially when the object structure is much more complex. We thus conduct registration~\cite{Zhou2018} between the general shape of the proposal and the template. Specifically, we sample 20\% points uniformly across the interval for the template and the proposal respectively, and then calculate the transform matrix between them by the ICP registration tool ~\cite{Zhou2018}. The template point cloud is registered according to the transform matrix.




% for each organ (\emph{i.e.}, kidney, liver), we first transform the template organ into the point cloud by the gridding reverse~\cite{xie2020grnet}. The point cloud template, denoted as $\mathbb{T}$, further serves as the supervision in the training of the \textit{mask head}. It provides better geometric supervision than previous height and width supervision~\cite{tian2021boxinst}. 

% **both proposal and template -> pc
% **introduce gridding reverse & 1-2 sentences why
% **introduce register & 1-2 sentences why
% then measure dis

\textbf{Loss} The geometric prior is then applied in the loss function of the \textit{mask head} training that we optimize the Chamfer Distance between the proposal $\mathbb{S}$ and the registered template organ $\mathbb{T}$. This can be formulated as follows:
\begin{equation}
\begin{aligned}
\label{eq:geo}
    L_{\text{geo}} =  \frac{1}{|\mathbb{S}|}\sum_{x\in \mathbb{S}}\min_{y\in \mathbb{T}}||x-y||_2 + \frac{1}{|\mathbb{T}|}\sum_{y \in \mathbb{T}}\min_{x\in \mathbb{S}}||y-x||_2.
\end{aligned}
\end{equation}
Specifically, the mask head produces binary segmentation masks for each proposal. The proposal is a probabilistic segmentation mask consisting of the segmented instances. This segmentation mask is further processed by the Gumbel-Softmax~\cite{jang2016categorical} to obtain the binary voxel. Locations of low probability are assigned to $0$ and vice versa. We then adopt the gridding reverse~\cite{xie2020grnet} to obtain the point cloud proposal $\mathbb{S}$ from the binary voxel. Finally, we calculate the Chamfer Distance between $\mathbb{S}$ and $\mathbb{T}$ as the geometric prior loss.




\subsection{Contrastive Similarity}
 Gray space performs poorly for the artifacts in medical imaging and similar surrounding tissues. It is not enough to distinguish between positive and negative pixels ({\em, i.e.}, organ pixels and non-organ pixels). We thus leverage contrastive learning to calculate the contrastive similarity between pixels. Encoding pixels to high-dimensional features and encouraging pixels of the same label to gather around in the embedding space helps to increase the distinguishability. 
%  in addressing the issues by artifacts in medical images, \emph{i.e.},  artifacts in ultrasound imaging and similar surrounding tissues. 
 
%  In the following paragraphs, we will first introduce the architecture and the training of the contrastive head, then discuss the overall contrastive similarity training scheme.

% training->loss: both geo and cs

% first pre-training, then loss

% Algorithm: first introduce contrastiev head,
% why build graph, then graph,
% then calculate similarity
% then introduce loss

To calculate the proposed contrastive similarity, we first build a ConvNet \textit{contrastive head} after the decoder. Following previous contrastive learning works~\cite{chen2020simple, hu2021semi}, we build a two-layer point-wise convolution $h(\cdot)$ to extract distinct representations from feature maps $P$. More specifically, we first pre-train the proposed \textit{contrastive head} in a coarse-to-fine fashion where only bounding box annotations are included in the pre-training stage. We encode pixels into embedding features $\mathcal{C}=h(P)$ and encourage pixels of the same label to gather around in the embedding space. The contrastive similarity between two pixels is defined as the distance in the embedding space. To calculate the contrastive similarity loss for the whole image, an undirected graph is constructed where the vertices correspond to the pixels and edges are links between neighboring pixels. The contrastive similarity associated with each edge is then summarized for the calculation of the overall contrastive similarity loss. Below we first introduce the pre-training of the contrastive head and then the definition of contrastive similarity loss.


%Then we utilize the high-dimensional features to build an undirected graph on the input image where vertices are pixels in the input image. And we define the label on the edg linking two points as \{0, 1\} by their distance in the embedding space. This is to distinguish organ pixels from non-organ pixels by their corresponding distance in the embedding space.


\textbf{Pre-training} The pre-training of the contrastive head is conducted in a weakly-supervised fashion that only bounding box annotations are included in the pre-training stage. To be more specific, there are two sub-stages in the pre-training stage: {\em coarse} and {\em refine}. In the {\em coarse} stage,
we first take pixels within the bounding box as positive labels and pixels outside the bounding box as negative labels. Then we train the contrastive head by such labeling. 
However, the performance of the contrastive head is largely limited for the noisy labels. Thus, we propose the {\em refine} stage to further improve the performance of the contrastive head.
In the {\em refine} stage, we first take random $K$ negative pixels as {\em referring pixels}. And for each pixel within the bounding box, we calculate the distance $\mathcal{D}$ between all K referring pixels:
\begin{equation}
\begin{aligned}
\label{eq:cons}
    D_{u, v, z} = \sum_{i=1}^{K}{\mathbbm{1}\{\{\mathcal{C}_{u,v,z} \cdot \mathcal{C}_{i}\}\geq \tau\} }
\end{aligned}
\end{equation}
where $\mathcal{C}_{u,v,z}$ $\in$ $R^{S \times H \times W}$ indicates the feature at the $(u, v, z)$ of the embedding features, $\mathbbm{1}$ stands for 1 if the distance is greater than $\tau$ and 0 if less, and $\tau$ is the threshold to decide whether pixels are positive or negative. If $D_{u, v, z}$ is greater than $K/2$, the pixel at location $(u, v, z)$ is considered positive, and vice versa. Then, we train the contrastive head using the same training loss as in the {\em coarse} stage, which is formulated as:
% If over K/2 referring pixels are 
% collect a random training sample with pixel-wise annotations. Then according to the pixel-wise annotations, organ pixels are assigned with positive labels and non-organ (\emph{i.e.}, background) pixels are assigned with negative labels. By encouraging pixels of the same label to gather around in the embedding space, the training loss of the \textit{contrastive head} can be formulated as:
\begin{equation}
\begin{aligned}
\label{eq:cons}
    loss= -\frac{1}{\left | \Omega \right |}\sum_{(u, v, z) \in \Omega}\frac{1}{\left | \mathcal{P}(u, v, z) \right |} \cdot
    ~~~~~~~~~~~~~~~~~~&\\
    ~~~~log\frac{\sum_{(u_p, v_p, z_p) \in \mathcal{P}(u, v, z)}exp(\mathcal{C}_{u ,v, z}\cdot \mathcal{C}_{u_p, v_p, z_p}/\tau )}{\sum_{({u}_{n}, {v}_{n}, {z}_{n}) \in \mathcal{N}(u, v, z)}exp(\mathcal{C}_{u, v, z}\cdot \mathcal{C}_{{u}_{n}, {p}_{n}, z_n}/\tau)}
\end{aligned}
\end{equation}
where $\mathcal{C}_{u,v,z}$ $\in$ $R^{S \times H \times W}$ indicates the feature at the $(u, v, z)$ of the feature map, and
$\Omega$ stands for {all points inside input}. %the points used in the calculation, 
$\mathcal{P}(u, v, z)$ denotes the set of points with the same label as the pixel at $(u, v, z)$  and $\mathcal{N}$ denotes the set of points with different labels. $\tau$ is the temperature constant.

\textbf{Loss} Considering an undirected graph $G=(V, E)$ built on the input image $I$, where $V$ corresponds pixels and $E$ indicates edges between neighboring pixels, the predicted segmentation mask can be viewed as the probability of pixel $(u, v, z)$ being foreground. Then the probability of pixel $(u_1, v_1, z_1)$ and pixel $(u_2, v_2, z_2)$ being the same label is: 
\begin{equation}
\label{eq:prob}
\begin{aligned}
Prob(y_e = 1) = \tilde{\mathcal{M}}_{u_1, v_1, z_1}
     \cdot
     {\tilde{\mathcal{M}}}_{u_2, v_2, z_2} 
     ~~~~~~~~~~~~&~~~~~~~~~~~~\\~~~~~~~~~~~~~~~+ (1 - {\tilde{\mathcal{M}}}_{u_1, v_1, z_1})     \cdot(1 - \tilde{\mathcal{M}}_{u_2, v_2, z_2}),
\end{aligned}
\end{equation}
where $\tilde{\mathcal{M}}$ indicates the foreground probability mask and $y_e$ represents the label of the edge.
% \qihua{what is $\tilde{M}$}

% we formulate the contrastive similarity as follows:
% \begin{equation}
% \label{eq:cons_sim}
% \begin{aligned}
% M_e = M(\mathcal{C}_{i, j}, \mathcal{C}_{l, k}) = \exp\left(-\frac{||\mathcal{C}_{i, j} - \mathcal{C}_{l, k}||}{\theta}\right),
% \end{aligned}
% \end{equation}
% where $M_e$ indicates the contrastive similarity of the edge $e$, and $\mathcal{C}_{i, j}$ and $\mathcal{C}_{l, k}$ are the contrastive vectors of the two locations $(i, j)$ and $(l, k)$ linked by the edge $e$, respectively. 
Thus, we can define an indicator on each edge to indicate whether they belongs to the same label. If the contrastive similarity between two neighboring pixels is above the pre-defined threshold $\tau$, the indicator on the edge linking them is assigned to $1$, and $0$ vice versa. We discard the edges with $0$ and further summarize the contrastive similarity loss of positive edges, which can be formulated as:
\begin{equation}
\label{eq:sim_loss}
\begin{aligned}
L_{\text{cons}} = -\frac{1}{N}\sum_{e \in E_{in}}\mathbbm{1}_{\{\mathcal{C}_{e_{start}} \cdot \mathcal{C}_{e_{end}} \geq \tau\}}\log Prob(y_e = 1).
\end{aligned}
\end{equation}
This serves as the contrastive similarity loss of the whole image.
%where $\mathbbm{1}_{\{\mathcal{C}_{e_{start}}\cdot \mathcal{C}_{e_{end}} \geq \tau\}}$ indicates 1 if the distance between two points is greater than the threshold $\tau$ and 0 otherwise.

% \textbf{Training loss} The contrastive similarity $M$ is calculated by a ConvNet \textit{contrastive head}. Following previous contrastive learning works~\cite{chen2020simple, hu2021semi}, we build a two-layer point-wise convolution $h(\cdot)$ to extract distinct representations from feature maps $P$. More specifically, we first calculate the contrastive similarity $\mathcal{C}$ as:
% \begin{equation}
% \label{eq:contrastive_sim}
% \begin{aligned}
% \mathcal{C}=\mathbbm{1}{\{h(P)\geq \tau\}}.
% \end{aligned}
% \end{equation}
% where $\mathbbm{1}$ indicates 1 if $h(P)$ is greater than the pre-defined threshold $\tau$, and 0 otherwise. 


% \begin{table*}[t!]
% \small
% \centering
% \scalebox{0.98}{
% \newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
% %\begin{center}
% % 	\begin{tabular}{c|P{1.65cm}P{1.3cm}P{0.8cm}P{1.1cm}P{0.7cm}P{0.8cm}P{0.9cm}|cccc}
% 	\begin{tabular}{c|cc|ccc|cc|cccc|c}
% 		\toprule[1.07pt]
% 		{\multirow{2}{*}{$\text{\#}$}} & BoxInst & DeeplabV3 & Gray &Cont. &SSIM  & ResNet & UNet & Weakly &   Fully & CPL & Internal & Dice$^\dagger$\\
% 		{} & Frame. & Frame. & Space & Sim. & Sim. & Backbone & Backbone & Supervised & Supervised & Head & Details &Score\\
% 		\midrule[1.07pt]
% % 		% baseline 
% % 		idx & boxinst & deeplab & gray & cont & ssim & resnet & unet & weakly & fully & cpl & internal & 49.3\\
		
% 		% weakly baseline
% 		1 & \checkmark &  & \checkmark &  &  &   & \checkmark & \checkmark &   &   &   & 49.3\\
% 		% +cont 
% 		2 & \checkmark &   &   & \checkmark &   &   & \checkmark & \checkmark &   &   &   & 56.8\\
% 		% +geo 
% 		3 & \checkmark &   &   & \checkmark &   &   & \checkmark &  \checkmark &   & \checkmark & \checkmark & 79.9\\
% 		% deeplab baseline 
% 		4 &   & \checkmark &   &   &   & \checkmark &   & \checkmark &   &   &   & 67.2\\
% 		% deeplab + geo_cont 
% 		5 &   & \checkmark &   & \checkmark &   & \checkmark &   & \checkmark &   & \checkmark & \checkmark & 76.9\\
% 		% resnet backbone  weakly
% 		6 & \checkmark &   &   & \checkmark &   & \checkmark &   &  \checkmark &   & \checkmark & \checkmark & 72.1\\
% 		% resnet backbone fully 
% 		7 & \checkmark &   &   &   &   & \checkmark &   &   & \checkmark &   &   & 91.7\\
% 		% unet backbone fully 
% 		8 & \checkmark &   &   &   &   &   &  \checkmark &   & \checkmark &   &   & 96.0\\
% 		% without cpl head 
% 		9 & \checkmark &   &   & \checkmark &   &   & \checkmark & \checkmark &   &   &  \checkmark & 79.1\\
% 		% without internal details 
% 		10 & \checkmark &   &   & \checkmark &   &   & \checkmark & \checkmark &   & \checkmark &   & 76.3\\
% 		% gray space 
% 		11 & \checkmark &   & \checkmark &   &   &   & \checkmark & \checkmark &   & \checkmark & \checkmark & 72.3\\
% 		% ssim space
% 		12 & \checkmark &   &   &   & \checkmark &   & \checkmark & \checkmark &   & \checkmark & \checkmark & 47.2\\
		
		
		
% 		\bottomrule[1.07pt]
% 	\end{tabular}
% }
% \caption{\small{Component-wise analysis. $\dagger$: we measure the corresponding dice score 



\begin{figure*}[htbp] 
	\centering
	\includegraphics[width=0.9\linewidth]{figs/method_only.pdf}
	\vspace{-0.7cm}
	\caption{The overall framework of our weakly-supervised segmentation framework with geometric prior and contrastive similarity. The training of our framework is organized as follows: We first pre-process the input images and obtain the embedding feature maps. Then we jointly supervise the mask head's training by the proposed geometric prior and contrastive similarity. In the aspect of geometric prior, we first convert the segmentation result to point cloud if complete. Then we calculate the Chamfer Distance between the result and the registered template. In the aspect of contrastive similarity, we first pre-train a contrastive head using only bounding box annotations. Then we minimize the distance between pixels of the same labels by the pre-trained contrastive head.}
	\label{fig:method} 
\end{figure*}


\begin{table*}[t!]
\small
\centering
\vspace{-0.3cm}
\caption{Performance comparison with other methods. We evaluate the performance using two metrics: Dice Score and HD95. $\dagger$ we obtain their dice score by their open source code. $\ddagger$: we rebuild the 3D framework based on its 2D open source code. {\em Ours w/o geometric} indicates we remove the geometric prior component. {\em Ours w/o contrastive} indicates we remove the contrastive similarity component.}
\renewcommand\arraystretch{1.4}
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
\resizebox{1.\linewidth}{!}{
    \begin{tabular}{P{4.3cm}P{2.7cm}P{1.3cm}P{1.3cm}cP{1.3cm}P{1.3cm}cP{1.3cm}P{1.3cm}}
        \specialrule{.8pt}{0pt}{2pt}
        \multirow{2}{*}{Method}  &  \multirow{2}{*}{Backbone} &
        \multicolumn{2}{c}{LiTS17}  && \multicolumn{2}{c}{KITS21}  && \multicolumn{2}{c}{LPBA40}  \\ 
        \cline{3-4}  \cline{6-7} \cline{9-10}
           &   &  $\uparrow$DSC(\%)&$\downarrow$HD95&&$\uparrow$DSC(\%)&$\downarrow$HD95  && $\uparrow$DSC(\%)  & $\downarrow$HD95  \\ 
          \specialrule{.4pt}{2pt}{0pt}
        %   \midrule[0.7pt]
          Fully Supervised & UNet~\cite{ronneberger2015u} & 95.5 & 5.3 && 96.0 & 3.2 && 83.7 & 2.1 \\
          \hdashline
          DeepCut (2016)~\cite{rajchl2016deepcut} & - & 37.1 & 15.2 && 36.2 & 14.7 && - & - \\
          SDI (2017)~\cite{khoreva2017simple} & VGG-16~\cite{simonyan2014very} & 49.2 & 11.7 && - & - && 38.7 & 9.0 \\
          
           MIL (2020)~\cite{Dolz2020}$^{\dagger}$  & ENet~\cite{paszke2016enet}& 69.4 & 9.4 && 72.3 & 8.7 &&- & - \\
           GMIL (2021)~\cite{hu2021semi}$^{\dagger}$  & ENet~\cite{paszke2016enet} & 71.1 & 8.8 && 71.7 & 5.9 && 58.2& 4.7\\
          
          BoxInst (2021)~\cite{tian2021boxinst}$^{\ddagger}$  &   UNet~\cite{ronneberger2015u} & 47.1 & 11.3 && 48.4 & 11.6 && 37.9 & 8.9\\
          \rowcolor[gray]{.95}
          Ours {\text{w/o geometric}} & UNet~\cite{ronneberger2015u} & {52.9}& {10.9} && {54.2} &{10.7}  && {44.9} & {7.1}\\
          \rowcolor[gray]{.95}
          Ours {\text{w/o contrastive}} & UNet~\cite{ronneberger2015u} & {69.7}&{9.4} && {68.5} &{9.1} && {57.3} & {4.9}\\
          \rowcolor[gray]{.9}
          Ours & UNet~\cite{ronneberger2015u} & \textbf{79.8} &\textbf{8.7} && \textbf{80.2}& \textbf{5.3} && \textbf{65.4} & \textbf{4.2}\\
        % \multicolumn{2}{*}{Multi-Column}
        % \midrule[1pt]
        % DeepCut~\cite{rajchl2016deepcut}  & TMI-16 & \CheckmarkBold  & bounding-box & \XSolidBrush & - & 37.1 & 36.2& - \\
        % % DeepCut~\cite{rajchl2016deepcut}  & - & \CheckmarkBold  & image-level & \XSolidBrush & & & & \\
        % SDI~\cite{khoreva2017simple}  & CVPR-17 & \CheckmarkBold  & bounding-box & \XSolidBrush & VGG-16 &- & - & -\\
        
        % BoxInst~\cite{tian2021boxinst}^{$\ddagger$}  & CVPR-22 & \CheckmarkBold  & bounding-box & \CheckmarkBold & UNet~\cite{ronneberger2015u} & 47.1 & 48.4 & 37.9\\
        % why not or why not on merge backbone, MIL~\cite{Dolz2020}^{$\dagger$}  & MIDL-20 & \CheckmarkBold  & bounding-box & \CheckmarkBold & UNet~\cite{ronneberger2015u}/ENet~\cite{paszke2016enet}& 69.4& 72.3 &- \\
        % why not or why not on mrege backbone, GMIL~\cite{hu2021semi}^{$\dagger$}  & MICCAI-21 & \CheckmarkBold  & bounding-box & \CheckmarkBold & UNet~\cite{ronneberger2015u}/ENet~\cite{paszke2016enet} & 71.1 & 71.7 & 58.2 \\
        % Ours & - & \CheckmarkBold & bounding-box  & \CheckmarkBold & UNet~\cite{ronneberger2015u} & \textbf{79.1} & \textbf{79.9} & \textbf{65.1}  \\ \cmidrule(lr){1-10}
        %  Fully Supervised & - & \XSolidBrush & ground-truth & \CheckmarkBold & UNet~\cite{ronneberger2015u} & 94.8 & 96.0 & 83.7 \\ 
        \specialrule{.8pt}{0pt}{2pt}
    \end{tabular}
}
\label{tab:main_res}
\vspace{-0.6cm}
\end{table*}



% remove venue, weakly, supervision, one-shot,
% dash line

% move fully-supervised to Line.1

% add tmi bbox




==> chap/related_works.tex <==
\section{Related Work}
\label{sec:related_work}
\IEEEPARstart{I}{n} this section, we first review existing weakly-supervised medical segmentation methods with bounding-box annotations in both natural and medical image segmentation, then we discuss recent works with geometric prior and finally present the trends in contrastive similarity.

% \subsection{Public medical semantic segmentation datasets}

% \subsection{Fully-supervised medical semantic segmentation}

% Medical semantic segmentation has been a challenge task for the irregular textures and arbitrary boundaries. To tackle these issues, U-Net~\cite{ronneberger2015u} adopts a symmetric encoder-decoder architecture with skip connections to gradually restore the downsampled feature maps to original size, thereby achieving pixel-level dense prediction of medical images. In the following research, U-Net based variants attract a lot of attention and are further applied in medical image segmentation. To fully utilize the local information among continuous slices which is also critical for volumetric segmentation,
% Cicek et al~\cite{cciccek20163d} generalize the U-Net from 2D
% to 3D by implementing 3D operations, such as 3D convolution
% and 3D max pooling, for better medical volumetric segmentation. To model long-range distance dependencies, Ozan Oktay~\cite{oktay2018attention} proposes a novel attention gate for medical
% imaging that automatically learns to focus on target structures
% of varying shapes and sizes. Based on the residual structure of
% ResNet ~\cite{he2016deep}, Residual U-Nets ~\cite{fang2019rca} are also proposed to overcome
% the difficulty in training deep neural networks.

\subsection{Weakly-supervised medical semantic segmentation}
Generally, methods in weakly-supervised segmentation are classified into four categories by the type of their weak annotations: scribbles~\cite{lin2016scribblesup}, points~\cite{bearman2016s, Qu2019}, image-level tags~\cite{patel2022weakly, Xu} and bounding-box annotations~\cite{kervadec2019constrained}. Scribbles and points supervision at least label one scribble or point for each region, and the annotated areas will be directly incorporated into the calculation of segmentation loss. Wang \emph{et al.}~\cite{wang2019weakly2} propose to leverage a random walker algorithm~\cite{Grady2006Random} to generate initial proposals for the unlabeled regions and then supervise the training of segmentation models by the initial segments. Qu \emph{{et al.}}~\cite{Qu2019} uses a similar training pipeline but a different label generation method for label generation which combines K-means clustering and Voronoi partition diagram. Xu \emph{et al.}~\cite{Xu} enrich the 
image-level labels to instance-level labels by multiple instance learning (MIL) and segment images using only volume-level labels.


% The major limitation of the aforementioned approaches is
% relying on additional dataset annotations, which can be time-consuming and is prone to errors 
% (for example, scribbles and points annotation can miss challenging labeled samples), and the errors can be propagated to the models during training. 

% % \subsection{Bounding box supervision}

Weakly-supervised segmentation with bounding box annotations earns increasing interest in medical image segmentation for its simplicity and low-annotation cost. We can define the bounding boxes with two corner coordinates that are easy to store in real scenarios. In addition, the bounding box annotations are location-aware so that they provide the spatial relationship of the target object, which is a popular direction in recent researches~\cite{dai2015boxsup,papandreou2015weakly,khoreva2017simple,pu2018graphnet}. In the early stages, researchers~\cite{papandreou2015weakly,rajchl2016deepcut} propose to consider pixels within the bounding box as foreground pixels and train the segmentation framework by these noisy labels. Despite the good performance achieved by such a scheme, they may accumulate errors during the alternative generation process. Most recently, researchers~\cite{tian2021boxinst} tried to directly generate the segmentation result instead of the error-prone alternative way. Generally, they build a {\em mask head} to produce the segmentation result, and the bounding box annotation is employed to train this mask head. 
In this work, we follow this segmentation scheme where the segmentation result is directly generated by the mask head. Furthermore, to address the fore-mentioned \qone\ and \qtwo\, we propose geometric prior and contrastive similarity, respectively.

\vspace{-0.2cm}
\subsection{Geometric prior}
Different from natural images, there exists obvious anatomical prior ({\em, i.e.}, atlas prior) in medical images, specifically in organs of human bodies (\emph{i.e.}, shape and position). Existing works incorporating such anatomical prior mostly fall into two categories: loss-based methods and graph-based methods. Generally, graph-based methods~\cite{patenaude2011bayesian, sabuncu2010generative, fischl2002whole, iglesias2015multi, gao2016segmentation} leverage the probability maps of occurring anatomy chances to construct graph models and estimate the foreground probability from the input image gray space. An appearance model of basic forms is employed to improve the segmentation accuracy~\cite{iglesias2015multi}. Gao {\em et al}~\cite{gao2016segmentation} proposes to apply an appearance ConvNet to characterize the foreground. Despite the high accuracy achieved by these methods, the graphical models bring heavy and expensive computational burdens to the segmentation framework, which makes it infeasible in certain scenarios. 

Another popular direction in combining the prior with the segmentation framework is loss-based methods. Researchers~\cite{ganaye2018semi, bentaieb2016topology, chen2017dcan, zhou2019prior, oktay2017anatomically, dalca2018anatomical} mostly minimize the distance between the segmentation network output and the pre-defined anatomical priors. Several works~\cite{ganaye2018semi, bentaieb2016topology} pose regularization terms on the training objective ({\em, i.e.}, anatomical adjacency or boundary conditions). Distance between predictions and atlas prior are also calculated in latent feature space~\cite{dalca2018anatomical, oktay2017anatomically}.

Compared with graph-based methods, loss-based methods provide a versatile fashion to incorporate anatomical priors with a wider range of scales while maintaining the computational efficiency of the segmentation framework. However, previous loss-based methods fail to address the aforementioned two issues for two aspects: 1) Previous works generally slice the volume into 2D or 3D patches, which are then processed sequentially to save memory cost. However, such a partitioning method breaks the global geometric relationships, resulting in inferior segmentation performance. Different from them, we learn the geometric prior in 3D embedding space to capture the overall geometry and proposed completeness head to ensure the shape completeness of
the proposal. 2) Unlike previous works using a volume representation, we leverage the Gridding Reverse~\cite{xie2020grnet} to convert the volume representation to point cloud representation. Compared to the volume representation constrained by uniform voxel grids, point cloud without grids is more flexible in representing delicate structures.


% Several works have been proposed in the fully-supervised framework to facilitate the network training by the geometric prior. A popular direction is to construct the statistical information about the spatial distribution of the organ in the medical images. Park {\em et al.}~\cite{park2003construction} seeks to construct a probabilistic atlas of four organs (\emph{i.e.}, liver, kidneys, and spinal cord) by 32 computed tomography (CT) scans and then leverage the calculated atlas to better segment low-contrast organs. Tong {\em et al.}~\cite{tong2015discriminative} leverages dictionary learning and sparse coding techniques to generate the statistical atlas which helps better automatically segment multiple organs. However, they suffer from the time-consuming post-processing based on the graph-cut methods. Zeng {\em et al.}~\cite{zeng2019liver} calculates the mean shape of the liver as the prior and generate the segmentation result based on the mean shape. ~\cite{huang2021medical} propose to facilitate the network training by incorporating the statistical information into loss function.
% Our method differs from previous work in two aspects: 1) The conventionally-used 2D embedding space indicates that they first slice the 3D input image into multiple 2D slices and then process these 2D slices sequentially to obtain the final result. Despite the light memory cost by such scheme, they fail to consider the spatial relationship between slices that the geometry of the specific organ is not well-preserved in their segmentation results. Different from the conventionally-used 2D embedding space, we learn the geometric prior in 3D embedding space which well preserve the 3D geometry of the specific organ. 2) Unlike previous works, we leverage the Gridding Reverse~\cite{xie2020grnet} to convert the volume representation to point cloud representation. The point cloud representation allows for the learning of more complex and difficult structures than volume representation.
% This helps better learn the spatial relationship between the segmentation result and the given organ template.

% for both contrastive similarity and geometrqic priro
% first survey: which method (volume or distane map or .....)
% then which point our mehthod should emphasize
% then ablation study design (other paper code & idea)
% (both fully , semi, weakly, key: volume )

% different from previously-used 2D embedding space, the geometric prior in our method is applied in 3D embedding space. This helps preserve the 

% The prior is not fully investigated in previous works~\cite{huang2021medical} that a 3D image is split into multiple 2D slices where the prior is introduced in these 2D slices. Instead, we apply the geometric prior in 3d space to guide the optimization of proposals by converting both geometric prior and proposals into point cloud.

% 2D break the shape, (ad: lack of 3d conssitency)

\vspace{-0.35cm}
\subsection{Contrastive learning}
Contrastive Learning aims to attract the positive and reverse the negative by dividing the feature space into positive and negative data pairs. As for semantic segmentation, it has been mainly used as pre-training~\cite{xie2020pointcontrast,xie2021propagate, he2020momentum}. Van \emph{{et al.}}~\cite{van2021unsupervised} apply it to distinguish features from various salient masks, showing its superiority in unsupervised set-ups. Wang \emph{{et al.}}~\cite{wang2021exploring} have shown advantages of contrastive learning by learning in both pixel
and region levels. Some researchers leverage contrastive learning to address the time-consuming pixel-wise labeling in medical image segmentation. Chaitanya \emph{et al.}~\cite{chaitanya2020contrastive} propose a two-stage
self-supervised contrastive learning framework to learn the feature matching both in global and local mechanisms from unlabeled data in the pre-training stage. Hu \emph{et al.}~\cite{hu2021semi} proposes a semi-supervised scheme to learn self-supervised global contrast and supervised local contrast. In our work, we observe that the conventionally-used gray space is not enough to distinguish positive and negative pixels ({\em, i.e.}, organ pixels and non-organ pixels), especially in Magnetic Resonance Imaging. We thus leverage contrastive learning to calculate the contrastive similarity between pixels. By encoding pixels to high-dimensional features and encouraging pixels of the same label to gather around in the embedding space, it enhances the discriminability and thus alleviates the poor performance of the gray space in handling medical imaging artifacts, \emph{i.e.},  artifacts in ultrasound imaging and similar surrounding tissues. 

% The conventionally widely-used gray space often perform poorly in medical segmentation that it is not robust enough to address the issues by artifacts in medical images, \emph{i.e.},  artifacts in ultrasound imaging and similar surrounding tissues. 

% contrastive learning->  cont sim -> our why
% because ad, thus we -> address xx issue


% The main difficulty
% of this approach is that an object may be segmented
% into multiple regions, some of which may merge it with
% its background. 

% Prior to deep learning approaches to automated image segmentation, techniques based on edge detection [6],
% region growing [7], contour modelling [8], and texture analysis [9] relied on detecting statistical difference
% among objects in an image using explicitly defined constraints and criteria. These methods can often perform
% pooly in medical imaging applications because typically used metrics, such as contrast gradients, are not
% robust enough to overcome the challenges imposed by noisy images, e.g., in ultrasound imaging, and artifacts,
% e.g., surrounding tissues.

